Decoding with Limited Teacher Supervision Requires Understanding When to Trust the Teacher

How can small-scale large language models (LLMs) efficiently utilize the supervision of LLMs to improve their generative quality? This question has been well studied in scenarios where there is no restriction on the number of LLM supervisions one can use, giving birth to many decoding algorithms that utilize supervision without further training. However, it is still unclear what is an effective strategy under the $\textit{limited supervision}$ scenario, where we assume that no more than a few tokens can be generated by LLMs. To this end, we develop an algorithm to effectively aggregate the small-scale LLM and LLM predictions on initial tokens so that the generated tokens can more accurately condition the subsequent token generation by small-scale LLM only. Critically, we find that it is essential to adaptively overtrust or disregard the LLM prediction based on the confidence of the small-scale LLM. Through our experiments on a wide range of models and datasets, we demonstrate that our method provides a consistent improvement over conventional decoding strategies. $\small$ $\textbf{Code:}$ https://github.com/HJ-Ok/DecLimSup

==> latex/table/llm_dataset_stat.tex <==
\begin{table*}[h]
\vspace{0.25cm}
\centering
\begin{tabu} to \textwidth { X[2,l]X[1,c]X[6,l] }
\hline
\textbf{Dataset} & \textbf{N} & \textbf{Example problem} \\ \hline
GSM8K & 1,319 & Josh decides to try flipping a house. He buys a house for \$80,000 and then puts in \$50,000 in repairs. This increased the value of the house by 150\%. How much profit did he make? \\ \hline
MultiArith & 420 & The school cafeteria ordered 42 red apples and 7 green apples for students lunches. But, if only 9 students wanted fruit, how many extra did the cafeteria end up with? \\ \hline
MATH & 5000 & What is the degree of the polynomial $(4 +5x^3 +100 +2\pi x^4 + \sqrt{10}x^4 +9)$? \\ \hline
ARC-Challenge & 1172 & An astronomer observes that a planet rotates faster after a meteorite impact. Which is the most likely effect of this increase in rotation?  Answer Choices: (A) Planetary density will decrease. (B) Planetary years will become longer. (C) Planetary days will become shorter. (D) Planetary gravity will become stronger. \\ \hline
ARC-Easy & 2376 & Which piece of safety equipment is used to keep mold spores from entering the respiratory system?  Answer Choices: (A) safety goggles (B) breathing mask (C) rubber gloves (D) lead apron \\ \hline
StrategyQA & 687 &Was ship that recovered Apollo 13 named after a World War II battle? \\ \hline
\end{tabu}
\caption{Summary of benchmarks we use in this paper with examples. \textit{N}: number of evaluation examples.}
\label{table:llm_dataset_stat}
\end{table*}
